Wheeler: A Three-Wheeled Input Device for Usable, Efficient, and Versatile Non-Visual Interaction

Blind users rely on keyboards and assistive technologies like screen readers to interact with user interface (UI) elements. In modern applications with complex UI hierarchies, navigating to different UI elements poses a significant accessibility challenge. Users must listen to screen reader audio descriptions and press relevant keyboard keys one at a time. This paper introduces Wheeler, a novel three-wheeled, mouse-shaped stationary input device, to address this issue. Informed by participatory sessions, Wheeler enables blind users to navigate up to three hierarchical levels in an app independently using three wheels instead of navigating just one level at a time using a keyboard. The three wheels also offer versatility, allowing users to repurpose them for other tasks, such as 2D cursor manipulation. A study with 12 blind users indicates a significant reduction (40%) in navigation time compared to using a keyboard. Further, a diary study with our blind co-author highlights Wheeler's additional benefits, such as accessing UI elements with partial metadata and facilitating mixed-ability collaboration.

==> sections/design_motivation.tex <==

% UI elements in modern applications and web pages are rich, interactive, and carefully designed with a combination of spatial location and typographic cues, such as hierarchy, font face, color, whitespace---all to create semantic relationships between different pieces of information on the screen~\cite{table-view2}.
% These semantic relationships are easy to comprehend by human visual perception. Consequently, sighted users can easily perceive and interact with the onscreen UI elements using a point and click device (e.g., a computer mouse) or directly via touch gestures.

% Unfortunately, this perceptual affordance of graphical UIs fundamentally differs for people with vision impairments who interact with computers non-visually using assistive technologies like screen readers~\cite{visual-non-visual-semantics}. 
% 
% For example, Boyd et al.~\cite{three-challenges} reported three challenges for blind users: (i) the pixel barrier, i.e., pixel-values and their location are not accessible to screen readers; (ii) mouse barrier, i.e., blind users cannot use a mouse, as it provides \emph{visual feedback} through a cursor; and (iii)  graphics barrier, i.e., difficulties in reconstructing visual semantics mentally.
%
% Screen readers, such as NVDA~\cite{NVAccess38:online}, JAWS~\cite{jaws_screenshade}, and VoiceOver~\cite{voiceover_osx}, despite being improved significantly over the years, fall short on addressing these challenges. As such, non-visual interaction with screen readers remains inefficient, cumbersome, and error-prone~\cite{vi_difficulties, Billah_ubiquitous}.

% A typical blind-sighted remote learning scenario would involve the blind users sharing their screen while a sighted confederate asks them to do certain tasks. These tasks may involve tracking a target on the screen, going to a certain menu option in a complex hierarchy, or mark objects in a shared document---all of which require spatial awareness of the screen contents from both sides. While a sighted confederate can see the blind user's screen and give proper instructions accordingly, the blind users have no choice but to rely on screen readers to act according to those instructions. But as screen readers creates their own manifest interfaces and loses the original spatial information on the screen, following the instructions become very hard if not impossible for the blind users.  
% 


To address the aforementioned problems, prior research proposed new rotary input devices such as \textit{Speed-Dial}~\cite{Billah_speeddial} and \textit{NVMouse}~\cite{haena-speeddial2}, to replace keyboard-only use of apps and websites.

% 
In Speed-Dial~\cite{Billah_speeddial}, Billah et al. used a rotary input device (e.g., a Surface Dial~\cite{surface_dial}) to interact with web pages and demonstrated that blind participants took significantly less time in performing data look-up and data comparison tasks using that rotary input, compared to screen-readers-provided keyboard-based navigation. %
Furthermore, they preferred the rotary input device because of its simpler and smaller gesture-sets (e.g., rotates and presses), compared to numerous keyboard shortcuts provided by screen readers, which are hard to memorize and easy to mix-up~\cite{Billah_ubiquitous}. 
% 
In addition, most blind participants associated these simpler gestures with mouse actions, e.g., \textit{rotations} with \textit{cursor movement} and \textit{presses} with \textit{clicks}. 
% 
Subsequently, Lee et al. reported similar findings~\cite{haena-speeddial1, haena-speeddial2}. In their \textit{NVMouse} prototype~\cite{haena-speeddial2}, Lee et al. reappropriated a traditional mouse-wheel as the input device. 
They found that wheel-based interaction, such as rotating and pressing the mouse wheel, consistently outperformed the keyboard-based interaction in editing tasks on Microsoft Word.




% 




% Describe how WH is different and its novelty
\sysname{} leverages these rotation-and-press-based interaction paradigm. However, its design philosophy is fundamentally different from prior work (e.g.,~\cite{Billah_speeddial, haena-speeddial1, haena-speeddial2, Billah_steeringwheel}), as well as keyboard-based navigation offered by screen readers. 
Three key differences are: 



\textbf{First}, \sysname{} is designed to navigate subtree in a hierarchy (e.g., UI Tree or DOM). For this reason, instead of using one rotary wheel, we use three---each for a different level of hierarchy.

\textbf{Second}, \sysname{} enables access to visual semantics on the granularity of individual UI (e.g., its location, size, shape, and layout).
% 
Access to these visual semantics can enable blind users to interact with graphical UIs efficiently, collaborate with sighted confederates (e.g., exchanging instructions) effectively, and facilitate building their own visual artifacts (e.g., website and blogs)~\cite{visual-non-visual-semantics} easily.
% 
Of particular importance is collaborating with sighted confederates  due to the rise of remote learning~\cite{remote-learning} and services like remote sighted assistance, such as Aira~\cite{Aira} and BeMyEyes~\cite{bemyeyes}.
%
% To effectively collaborate, both sighted and blind individuals should have a shared understanding of the overall UI semantics and the focused UI element. 
% % 
% Unfortunately, screen readers cannot provide the full access to such visual semantics~\cite{visual-non-visual-semantics}. 
% \sysname{} is designed to fill this void. 

==> sections/extra_sections.tex <==
\begin{comment}

\section{Movement Time Mathematical Formulations}

\subsection{Acquiring Targets Using the Shortest Distance}

\begin{figure*}[!ht]
  \centering
  \includegraphics[width=.90\columnwidth]{figures/basic_fitts_modified.png}
  \caption{Acquiring Targets Using Shortest Distance}
  \label{fig:basic_fitts}
\end{figure*}


Let us consider the scenario presented in Figure~\ref{fig:basic_fitts}; where user is trying to move the cursor from the source to the target object.
%
Here, A is the distance between the source and the target, and W is the width of the target.
%
Jagacinski et al. \cite{jagacinski2018control} presented a derivation of required time for such a move using the first-order lag system of Control Theory. Here is how the formulation looks like:

\begin{equation}
\label{eq:mt_from_control_theory}
    t = \frac{\ln{(2)}}{k}\log_2{(\frac{2A}{W})}
\end{equation}

 
Where, k is called the gain factor, which determines the speed at which the target is acquired~\cite{jagacinski2018control}.

Equation~\ref{eq:mt_from_control_theory} is indeed another formulation of the Fitts' law~\cite{fitts1954information}. According to Fitts' law:


\begin{equation}
\label{eq:fitts_law_1}
    t = a + b * ID
\end{equation}

Where, ID stands for Index of Difficulty and,  
\begin{equation}
\label{eq:fitts_law_2}
    ID = \log_2{(\frac{2A}{W})}
\end{equation}



\subsection{Acquiring Targets Using Rectilinear Distances}


\begin{figure*}[!ht]
  \centering
  \includegraphics[width=.85\columnwidth]{figures/rectilinear.png}
  \caption{Acquiring Targets Using Rectilinear Movements}
  \label{fig:rectilinear}
\end{figure*}

In \sysname{}'s \fnav{} mode, users use rectilinear movements to go from source ($X_0$, $Y_0$) to target ($X_1$, $Y_1$). 
%
For example, In Figure~\ref{fig:rectilinear}, the users would travel the distances $A_1$ and then $A_2$, instead of only $A$ like sighted users usually do.
%
In this section, we try to formulate an equation for movement time using such movements. 

In this scenario, we can derive the movement times for $A_1$ and $A_2$ separately using Equation~\ref{eq:mt_from_control_theory}.
%
If $t_1$ and $t_2$ unit times are needed for traversing distances $A_1$ and $A_2$ respectively, we can write:

\begin{equation}
    t_1 = \frac{\ln{(2)}}{k}\log_2{(\frac{2A_1}{W})}    
\end{equation}

and, 

\begin{equation}
    t_2 = \frac{\ln{(2)}}{k}\log_2{(\frac{2A_2}{W})}    
\end{equation}

If total movement time in this case is $T_{rec}$, then, 

\begin{equation}
\label{eq:rectilinear_travel}
\begin{aligned}
        T_{rec} &= t_1 + t_2 \\
          &= \frac{\ln{(2)}}{k} [ \log_2{(\frac{2A_1}{W})} + 
          \log_2{(\frac{2A_2}{W})} ] \\
          &= \frac{\ln{(2)}}{k} [\log_2{(\frac{4A_1A_2}{W^2})}]
\end{aligned}
\end{equation}

Where, $A_1=|X_1-X_0|$ and $A_2=|Y_1-Y_0|$.


\subsection{Rectilinear Vs. Shortest Path Travel}

In Figure~\ref{fig:rectilinear}, If path $A$ was taken instead of \{$A_1$, $A_2$\} to reach the target, then the movement time $T_{shortest}$ would be:

\begin{equation}
\label{eq:shortest_path_travel}
    T_{shortest} = \frac{\ln{(2)}}{k}\log_2{(\frac{2A}{W})}
\end{equation}

From Figure~\ref{fig:rectilinear}, it is easy to see that $T_{shortest}$ is smaller than $T_{rec}$.
%
The following calculation shows the difference between $T_{rec}$ and $T_{shortest}$:

\begin{equation}
\label{eq:delta}
\begin{aligned}
        \Delta T  &= T_{rec} - T_{shortest} \\
        & = \frac{\ln{(2)}}{k} [\log_2{(\frac{4A_1*A_2}{W^2})}] 
        - \frac{\ln{(2)}}{k}\log_2{(\frac{2A}{W})}
        \\
        &= \frac{\ln{(2)}}{k} [\log_2{(\frac{4A_1*A_2}{W^2})} - \log_2{(\frac{2A}{W})}] \\
        &= \frac{\ln{(2)}}{k} [\log_2{(\frac{4A_1*A_2}{W^2}*\frac{W}{2A}})] \\
        &= \frac{\ln{(2)}}{k}[\log_2{(\frac{2A_1*A_2}{AW})}] \\
\end{aligned} 
\end{equation}
% \fx{Never end an equation without an explanation. Your equation is only usable if your explanation is good; otherwise, it adds no value to reader. For example, check out my addition below.}

Using the Pythagorean theorem, $A$ can be written in terms of $A_1$ and $A_2$ as follows: $\sqrt{A_1^2 + A_2^2}$. Therefore, Eq.~\ref{eq:delta} can be written as below:

\begin{equation}
\label{eq:delta2}
\begin{aligned}
        \Delta T  &= T_{rec} - T_{shortest} \\
        &= \frac{\ln{(2)}}{k}[\log_2{(\frac{A_1*A_2}{A}* \frac{2}{W})}] \\
        &= \frac{\ln{(2)}}{k}[\log_2{(\frac{A_1*A_2}{\sqrt{A_1^2 + A_2^2}}* \frac{2}{W})}] \\
        &= \frac{\ln{(2)}}{k}[\log_2{(\frac{1}{\sqrt{\frac{1}{A_1^2} + \frac{1}{A_2^2}}}* \frac{2}{W})}] \\
\end{aligned} 
\end{equation}

One can interpret the above Eq.~\ref{eq:delta2} as follows: 
\begin{itemize}
    \item If $A_1 \to 0$ or $A_2 \to 0$, i.e., the both the source and the target are parallel to X- or Y-axis, the difference in time for rectilinear and shortest movements reduces to zero ($\Delta T \to 0$).
    % 
    \item If $A_1 \to A_2$ or $A_2 \to A_1$, indicating the angle between X- or Y-axis and the line connecting the source and the target becomes 45 degrees, $\Delta T$ reaches its maximum value, i.e., $\frac{\ln{(2)}}{k}[\log_2{(\frac{A_1}{\sqrt{2}}* \frac{2}{W})}]$ or $\frac{\ln{(2)}}{k}[\log_2{(\frac{A_2}{\sqrt{2}}* \frac{2}{W})}]$.
    % 
    \item If one component is significantly larger than other, $A_1 >> A_2$, $\Delta T$ depends on the smaller component ($\Delta T \approx \frac{\ln{(2)}}{k}[\log_2{(A_2 * \frac{2}{W})}]$, assuming $\frac{1}{A_1^2} \to 0$).
\end{itemize}






\subsection{Rectilinear Travel at different Speeds}
\sysname{} has an option to modify the cursor speed (via the third wheel) in \fnav{} mode. This would enable the users to speed up the movements in rectilinear motions if they want to.
%
If the user speeds up the cursor movement by a factor of $s$ (\textbf{assuming s>1}), then the effective distances they have to travel become $\frac{A_1}{s}$ and $\frac{A_2}{s}$ instead of $A_1$ and $A_2$ respectively. 
%
If we call the movement time $T_{rec-speed}$ this time, Equation~\ref{eq:rectilinear_travel} becomes:

\begin{equation}
\label{eq:rectilinear_travel_speed}
\begin{aligned}
        T_{rec-speed}
          &= \frac{\ln{(2)}}{k} [ \log_2{(\frac{\frac{2A_1}{s}}{W})} + 
          \log_2{(\frac{\frac{2A_2}{s}}{W})} ] \\
          &= \frac{\ln{(2)}}{k} [ \log_2{(\frac{2A_1}{Ws})} + 
          \log_2{(\frac{2A_2}{Ws})} ] \\
          &= \frac{\ln{(2)}}{k} [\log_2{(\frac{4A_1A_2}{W^2s^2})}]
\end{aligned} 
\end{equation}

Now, let us consider that we pick $s$ in a way so that $T_{rec-speed}$ and $T_{shortest}$ becomes equal. In other words, we want to see how much we have to speed up (s) the movement to achieve shortest path (sighted) performance from the rectilinear path.

Hence,

\begin{equation}
\label{eq:deriving s}
\begin{aligned}
        & T_{rec-speed}
          = T_{shortest} \\
        &\implies \frac{\ln{(2)}}{k} [\log_2{(\frac{4A_1A_2}{W^2s^2})} =
        \frac{\ln{(2)}}{k}\log_2{(\frac{2A}{W})} \\
        &\implies \frac{4A_1A_2}{W^2s^2} = \frac{2A}{W} \\
        &\implies As^2W = 2A_1A_2 \\
        &\implies s = \sqrt{\frac{2A_1A_2}{AW}} \\
\end{aligned} 
\end{equation}

% \fx{So what? Explain how one can interpret the above equation}.

Where, $A_1=|X_1-X_0|$,  $A_2=|Y_1-Y_0|$, and $A=\sqrt{(X_1-X_0)^2 + (Y_1-Y_0)^2}$ 


Thus, if we have :

\begin{enumerate}
    \item the source ($X_0$, $Y_0$) and the target ($X_1$, $Y_1$) coordinates, and
    \item  the width of the target (W),
\end{enumerate}

we can determine how much speed increment in rectilinear movements is necessary to achieve the same performance as that of taking the shortest path.


\paragraph{\textbf{When s<1:}}
s=1 means we expect the speed in rectilinear movements to be the same as the shortest path movement.
%
However, with some users, the conditions s=1 or s>1 may not be achievable.
%
In \sysname{}'s \fnav{} mode, the third wheel also allows the users to slow down the cursor i.e., activate a scenario where s<1. 
%
When they do so, the movement time will be higher as indicated by Equation~\ref{eq:rectilinear_travel_speed}.  






\section{Computational Interaction}

Computational Interaction is concerned with abstracting, explaining, and enhancing the interactions between humans and systems via the use of algorithms, data, and mathematical models~\cite{oulasvirta2018computational}.
%
In the early days of human-system interaction, the design spaces were much simpler; and static input-to-output mappings used to be good enough for most devices (e.g., a TV remote, a switch, or a lock-and-key mechanism).
%
However, with modern complex and non-deterministic input-output mappings, designers often need to use probabilistic modelling, data-driven approaches, and Artificial Intelligence-based techniques such as Machine Learning.
%
% Working with and visualizing such complex techniques can result in cognitive overload, lack of proper understanding, and ultimately bad design choices from the designers. \fx{too broad, too high-level, thus contains 0 info. Provide short example in (e.g., ....)}
%
Working with such complex techniques (e.g., trying to understand a pattern in a dataset with hundreds of dimensions, identifying useful features while training a Machine Learning model, or dealing with an oversupply of information~\cite{kirsh2000few}) are next to impossible without the use of high-level visualization tools or summary statistics.
%
Computational interaction provides a systematic approach to this problem with useful techniques such as visualization, simulation, and automated evaluations.
%
The task of computational interaction is not to replace the human designers---but to augment their capabilities in making informed decisions regarding what is and what is not a good choice for a specific interaction~\cite{oulasvirta2018computational}.


%\fx{if there are so many models, why control theory (CT) in particular? Ans: think of what's so unique about CT  that others don't have?}.
%


Computational Interaction builds upon an arsenal of tools, theories, and methods including but not limited to information theory, probabilistic modelling, machine learning, optimization, rationality, and control theory~\cite{oulasvirta2018computational}.  
%
Among these, control theory~\cite{jagacinski2018control} is of special interest to HCI researchers as it helps modelling interaction as a continuous event---which is arguably the true nature of interactions~\cite{doherty1999continuous}.
%
At the center of control theory is a model named \emph{control system} with a feedback loop. 
%
Using such a model for designing interactions tackles the fundamental limitations of stimulus-response based approaches, which fails to incorporate feedback~\cite{oulasvirta2018computational}.
%
The control system (also known as control loop) is centered around the idea of minimizing error---the difference between the current and the desired state of an output, in response to an interaction.
%
Apart from human-controlled and system-controlled elements, modern control loops also account for the state of the controlled variable and external disturbances. 
%
While earlier Information Theory-based models such as Fitts' law~\cite{fitts1954information} can account for interactions only when the target is static, control loops can address and model moving targets, space-constrained movements, time-dependent motions, etc.
%
Moreover, as Jagacinski et al. have shown, Fitt's law equations can be derived from control theory and its components such as the first-order lag system~\cite{jagacinski2018control}.
%
This goes to show that when compared to information theory, Control Theory is the more general framework.
\fx{this write-up is so much better!! It paints a sharper picture. The readers can learn something interesting, which is the point of any related work section. Good job!!}

\subsection{Computational Interaction, Control Theory, and KB-Based Interaction}

% \fx{Another para on Control theory for modeling keyboard-based interaction, assistive technology (screen reader) interaction modeling? What is the current state, prior work, challenges, potential ideas for incorporation}


% \fixmeth{Not Final Yet, Accumulated important texts for now}


Previous research in Computational Interaction has focused mostly in optimizing the experience for sighted users, i.e., users who can observe and interact with the visual cues (e.g., moving target, different font-faces, text styles, spacing). 
%
However, little to no effort has been given in understanding and optimizing the interactions of Blind and Low-Vision (BLV) users from a computational interaction point of view.
%
This creates a discrimination because the improvements brought upon by computational interaction and its components such as control theory are available to users based on their abilities such as sight.
%
In this section, we look at how we can model non-visual, keyboard-based, and screen reader-assisted interactions using control theory and its different components.

The first step to modeling an interaction with a control system is to make sure that the interaction in consideration is continuous. 
%
In other words, there must be a continuous signal loop between the user and the interface, and the user should continuously be attempting to minimize the error between his/her intention and the system's current state~\cite{oulasvirta2018computational}.
%
The purpose of the aforementioned loop is to incorporate feedback---allowing the user to understand how far they are from their destination.
%
The loop also also takes care of any external disturbances or noises by changing modifying the controlled variables and thereby notifying the user.






To model non-visual, keyboard-based interactions using control theory, we need to address the aforementioned points. To put simply, we need the interaction between the system and the user to be continuous, we need a feedback loop, and a mechanism to address external disturbances and errors by the user.
%
In this research, we focus on keyboard-based (and screen reader assisted) navigation only as this poses the primary challenge for users with visual impairments according to our experience.
% 
A typical navigation scenario is presented in Figure~\ref{fig:ms_word} and~\ref{fig:hierarchy_ms_word}.
% 

% \fixmeth{The next two paras are repeated section 12, but that is a different topic, and may go to a different paper. So, we are good for now.}
Shown in Figure~\ref{fig:ms_word} is a screenshot of Microsoft Word; a BLV user is using a screen reader (SR) and keyboard arrow keys to get from the \texttt{Home} ribbon option (marked with number 1, boxed in a green rectangle) to the \texttt{Right Align} option (marked with number 6).
%

Figure~\ref{fig:hierarchy_ms_word} illustrates all the possible valid transitions when using the arrow keys for this scenario.
%
From Figure~\ref{fig:hierarchy_ms_word}, it is easy to see that the user would have to take the path $1\xrightarrow{}2\xrightarrow{}3\xrightarrow{}4\xrightarrow{}5\xrightarrow{}6$.
%
Here, the move $1\xrightarrow{}2$ is performed using the down arrow ($\downarrow{}$) key and the rest are performed using the right arrow ($\rightarrow{}$) key.


We need to model this navigation using a control system. 
%
There are three ways a BLV user can perform the navigation shown in Figure~\ref{fig:ms_word}:

\begin{enumerate}
    \item \textbf{Case 1: Brute force approach, i.e., user does not know the path}
    
    \item \textbf{Case 2: Optimal way, i.e., user knows/is given the path}
    
    \item \textbf{Case 3: User uses screen reader shortcuts/search options.} In this case, the user searches for the target object by its label/class. Then the SR makes a 1D list of all the UI objects with that label. As such, the user can navigate the list in a linear fashion until they find their target.
    
\end{enumerate}

\paragraph{\textbf{Control Task:}} In all three cases, the control task for the user is to reach the target object in the UI.


\paragraph{\textbf{Error Metric:}} This is the metric that the user will be attempting to minimize continuously until they reach their targets. 
%
One option for the error metric would be the minimum number of steps (i.e., keystrokes) required to reach the target from the current position of the keyboard focus.
%

For example, in Figures~\ref{fig:ms_word} and~\ref{fig:hierarchy_ms_word}, the user's optimal path from start to destination is: $1\xrightarrow{}2\xrightarrow{}3\xrightarrow{}4\xrightarrow{}5\xrightarrow{}6$.
%
The following table shows the user's position at different stages and the values of the error metric at that position.
%
\begin{center}
\begin{table}[!ht]
\begin{tabular}{| c| c| c |}
\hline
 \textbf{Current Position} & \textbf{Remaining Path to Destination} & \textbf{Remaining Cost (Error Metric)}  \\ \hline
 1 & $1\xrightarrow{}2\xrightarrow{}3\xrightarrow{}4\xrightarrow{}5\xrightarrow{}6$ & 5 \\  \hline
 2 & $2\xrightarrow{}3\xrightarrow{}4\xrightarrow{}5\xrightarrow{}6$ & 4 \\  \hline
 3 & $3\xrightarrow{}4\xrightarrow{}5\xrightarrow{}6$ & 3 \\  \hline
 4 & $4\xrightarrow{}5\xrightarrow{}6$ & 2 \\  \hline
 5 & $5\xrightarrow{}6$ & 1 \\  \hline
 6 & - & 0 \\  \hline
\end{tabular}
\caption{Different travel positions in the navigation task shown in Figures~\ref{fig:ms_word} and~\ref{fig:hierarchy_ms_word}, along with their respective remaining paths and error metrics. As the user gets closer to the target, the error metric gets smaller.}
\label{table:error_metrics}
\end{table}
\end{center}


\paragraph{\textbf{Feedback:}}
For visual navigation, the user can see the cursor moving on the screen as per their commands via mice, joysticks, or trackpads.
%
The user uses the change in cursor position on the screen as a feedback and adjusts their subsequent movements accordingly.
%
For non-visual navigation, the feedback comes primarily from the screen reader's audio output.
% 
As the screen reader reads relevant information regarding the current input in focus, the user listens to them and decides whether they are moving towards or away from their target.
%

In case 1, there is no way for the user to understand/calculate how far they are from the target.
%
As such, the screen reader audio cannot serve as the feedback as it does not help the user to minimize the error in subsequent movements.

%
In case 2, the user knows the path, i.e., the intermediate objects the path consists of. As such,
the user can verify each intermediate object in the path by listening to the screen reader. 
%
In the case of a wrong move, the user would know that immediately and backtrack to get back on the correct path.
%

In case 3, the user is basically going through a 1D list of all the objects that have the target label. Thus, the user listens to the SR and decides if they are already at their target object or not. If not, the user continues navigating the 1D list.



\paragraph{\textbf{External Noise and Disturbances:}}
External noises and disturbances may come from wrongly pressing a key, screen reader malfunctions, and lack of accessibility in an application or website.
%
User errors are addressed through the use of feedback---if the user presses a wrong key, the SR output will not be what they expect.
%
Screen reader malfunctions can be addressed by closing and restarting the screen reader. There are shortcuts that allow users to perform this task.
%
While lack of accessibility in an app or website cannot be solved, it can at least be identified.
%
When an element in the UI is inaccessible, the SR usually stays quiet despite a key-press or says "blank, blank".



% \begin{itemize}
%     \item If we can identify a continuous signal loop between the user and interface, such that the user is, at times, continuously minimizing the error between his or her intention and the system state, we can say the user is interacting in a continuous fashion with the system.
    
%     \item The control loop attempts to minimize error. Thus, if we can formulate the error function, we can model any interaction with Control Theory (CT).
    
%     \item Very little focus has been given to keyboard (and hence screen reader) based interactions in the field of computational interaction, or control theory.
    
%     \item Goal: Putting SR-based interactions on the same level of importance as other modes.
    
%     \item Goal: Utilizing the well-established models and tools in control theory to advance the state of SR-based interactions.
    
%     \item Goal: Quantification of accessibility
    
% \end{itemize}



\begin{figure*}[!ht]
  \centering
  \includegraphics[width=.85\columnwidth]{figures/control_loop.png}
  \caption{A control loop showing the components for designing keyboard-based interactions.}
  \label{fig:control_loop}
\end{figure*}





Figure~\ref{fig:control_loop} shows all the components of the control system we are proposing to address keyboard-based, non-visual, SR-assisted navigation.
%
Note that the control system here contains only human control as opposed to a combination of human and computer controls as shown by Oulasvirta et al. ~\cite{oulasvirta2018computational}.
%
We propose it this way because computers can do little with the SR's audio output.
%
The human auditory system, on the other hand, can comprehend and act accordingly listening to such feedback. 
%
External noises or errors can change the current keyboard focus (i.e., the controlled variable). However, the user should be aware of this via SR's audio output.







\section{Determining Keyboard-based Navigation Times Using GOMS and KLM Models}
% \fixmeth{collecting info}

\emph{Goals, Operators, Methods, Selection Rules}, otherwise known as GOMS~\cite{card2018psychology}, is an engineering model commonly used for abstracting and comparing early designs.
%
First, the model breaks down each task into atomic-level micro-tasks, then handles the micro-tasks, and finally returns to the original task with cumulative results in a bottom-up fashion.
%
By atomic level, the model understands tasks that are recognizable and comprehensible; and whose difficulty can be expressed in terms of some predefined quantitative metric such as execution time in seconds.
%
Such breakdowns are necessary to understand the difficulty (i.e., physical effort, execution time) of performing a certain high-level task.
%
An example of such a high-level task would be navigating to a certain option (e.g., a text, an image, a checkbox) in a specific User Interface (UI).
%
GOMS makes it possible to calculate the completion time of such tasks~\cite{tonn2006measuring}, as well as full-scale analysis of UIs~\cite{john1996using, john1996goms} for comparison.  
%
GOMS also paves the way for using other models such as KLM (keystroke-Level Model)~\cite{card1980keystroke}.


KLM estimates the task execution time for specific scenarios in a given design~\cite{kieras2001using}.
%
Similar to GOMS, KLM requires a high-level task to be broken up until the point where each sub-task can be accomplished using one or more predefined operators (either physical or mental).
%
For keyboard-based navigation, the physical operator is a keystroke. 
%
The required time for each keystroke is then estimated, along with any delays for the user to think (i.e., mental operator).
%
Different atomic-level tasks and their estimated execution times are available in Kieras et al.'s work~\cite{kieras2001using}.
%
Here is a summary of the operators that will be necessary in our analysis along with their execution times:

\begin{center}
\begin{table}[!ht]
\begin{tabular}{| c| c| c |}
\hline
 \textbf{Operator} & \textbf{Operator Symbol} & \textbf{Estimated Execution Time (s)}  \\ \hline
 1. Keystroke & K & 0.12-1.2 (0.28 Recommended) \\  \hline
 2. Mental act of routine thinking & M & 0.6-1.35 (Recommended 1.2)    \\\hline
 3. Waiting for the System to respond  & W(t) & 0.1 (\fixmeth{assumption}) \\ \hline
 4. Screen Reader Reading Item Name & S(n) & 0.5 (\fixmeth{assumption})\\ \hline
 5. Screen Reader Reading Item Label & S(l) & 0.3 (\fixmeth{assumption}) \\ \hline
\end{tabular}
\caption{Different operators with their estimated execution times. Items 1-3 are collected from Kieras et al.'s work~\cite{kieras2001using}. Items 4 and 5 are estimated according to our experience of working with assistive technology users.}
\label{table:operator_times}
\end{table}
\end{center}






\subsection{Using KLM to Estimate Movement Time in Keyboard-based Navigation}

One very common use-case for the BLV people is to perform navigation (i.e., going from one UI item to another) on a UI using the combination of screen readers (e.g., NVDA~\cite{nvda}, JAWS~\cite{jaws}, VoiceOver~\cite{voiceover_osx}) and keyboards.
%
In such a scenario, the user uses the arrow keys (i.e., up, down, left, right) in the keyboard to move the focus from one item to another.
%
When the focus moves, the screen reader reads out some information (usually name and label) regarding the item currently in focus.
%
The user listens to the screen reader sound output and evaluates if the current item in focus is indeed the item the user wishes to get to.
%
Now, let us consider a navigation scenario and determine the time required for such an action using the ideas from KLM and GOMS models.





\paragraph{\textbf{Scenario}} 
Shown in Figure~\ref{fig:ms_word} is a screenshot of Microsoft Word; a BLV user is using a screen reader (SR) and keyboard arrow keys to get from the \texttt{Home} ribbon option (marked with number 1, boxed in a green rectangle) to the \texttt{Right Align} option (marked with number 6).
%

Figure~\ref{fig:hierarchy_ms_word} illustrates all the possible valid transitions when using the arrow keys for this scenario.
%
From Figure~\ref{fig:hierarchy_ms_word}, it is easy to see that the user would have to take the path $1\xrightarrow{}2\xrightarrow{}3\xrightarrow{}4\xrightarrow{}5\xrightarrow{}6$.
%
Here, the move $1\xrightarrow{}2$ is performed using the down arrow ($\downarrow{}$) key and the rest are performed using the right arrow ($\rightarrow{}$) key.


\begin{figure*}[!ht]
    \begin{minipage}{.45\linewidth}
      \centering
      \includegraphics[width=\columnwidth]{figures/word.png}
      \caption{A screen capture of MS Word, with a few clickable elements labeled with numbers.}
      \label{fig:ms_word}
      \end{minipage}
      \hspace{.05\linewidth}
      \begin{minipage}{.45\linewidth}
      \centering
             \begin{tikzpicture}[node distance={15mm}, thick, main/.style = {draw, circle}] 
    
        \node[main] (1) {$1$}; 
        \node[main] (3) [below left of=1] {$3$}; 
        \node[main] (2) [left=.5cm of 3] {$2$}; 
        \node[main] (4) [below=.5cm of 1] {$4$}; 
        \node[main] (5) [below right of=1] {$5$}; 
        \node[main] (6) [right=.5cm of 5] {$6$}; 
        \draw[<->] (1) -- (2); 
        \draw[<-] (1) -- (3); 
        \draw[<-] (1) -- (4); 
        \draw[<-] (1) -- (5); 
        \draw[<-] (1) -- (6); 
        \draw[<->] (2) -- (3); 
        \draw[<->] (3) -- (4); 
        \draw[<->] (4) -- (5); 
        \draw[<->] (5) -- (6); 
        
        
        \end{tikzpicture}  
        \caption{A simplified DOM representation of the labeled UI elements in Figure~\ref{fig:ms_word}.  The Home ribbon tab is a parent of the other elements, which are siblings in the hierarchy.}
        \label{fig:hierarchy_ms_word}
      \end{minipage}
\end{figure*}

\paragraph{\textbf{Assumptions}}
We assume that the user is expert (which is also a primary assumption and a limitation of GOMS model~\cite{tonn2006measuring}) and knows the navigation path from the source to the target.
%
We also assume that the user knows the name (e.g., boldface, italic, right align) and label (e.g., button, text, image) of the target.

\paragraph{\textbf{Sequence of Operators}}
The following sequence illustrates the atomic level events/operators (along with their symbols) needed for us to apply the KLM model and find the total navigation time.
The task breakdown is motivated by Tonn-Eichst{\"a}dt's work~\cite{tonn2006measuring}, which also calculates different task completion times in a website for screen reader users.

\begin{enumerate}
    \item Initiate the navigation from the \texttt{Source} (Decide to do the task) (\textbf{M})
    \item Press the next navigation key (\textbf{K})
    \item Wait for the SR to read out information on the current item in focus(\textbf{W(t)}) 
    \item The SR reads out the item name (\textbf{S(n)})
    \item The SR reads out the item label (\textbf{S(l)})
    \item Verify if the item name is the target name (\textbf{M})
    \textbf{[If negative, go to step 2]}
    \item Verify if the item label is the target label (\textbf{M})
    \textbf{[If negative, go to step 2]}
    \item Stop the navigation (\textbf{M})
\end{enumerate}

Using the above steps, we can determine the total time ($T$) required for the navigation described in the scenario in Figures~\ref{fig:ms_word} and ~\ref{fig:hierarchy_ms_word}.

\begin{equation}
\begin{aligned}
     T &= M + 4 * [ K + W(t) + S(n) + S(l) + M ] + K + W(t) + S(n)  + S(l) + M + M + M \\
       &= 8M + 5K + 5W(t) + 5S(n) + 5S(l) \\
       &= 8*1.2 + 5*0.28 + 5* 0.1 + 5*0.5 + 5*0.3 \\
       &= 15.5s
\end{aligned}
\end{equation}

Here, the first four navigation keystrokes do not take the user to the target.
%
For all of these, the sequence returns to step 2 from step 6.
%
For the final keystroke, however, all the steps from 2-8 are executed.



\paragraph{\textbf{Limitations}}
Below are some of the limitations associated with the approach above:

\begin{enumerate}
    \item We assumed error-free navigation; however, if a user presses a wrong arrow key, they may need significantly more time to get back on track, or to reach the destination.
    \item As suggested by Table~\ref{table:operator_times}, the execution times for T and M can vary widely depending on the user's capability. Hence, the above model only provides an estimate (possibly a lower bound) on the required navigation time.
    \item The operator execution times in Table~\ref{table:operator_times} is for all users. The data was not collected specifically for BLV people using assistive technologies.
\end{enumerate}


\end{comment}

==> sections/intro_extras.tex <==
\begin{comment}
An assistive technology-mediated, keyboard-only interaction is different from interacting with the two-dimensional (2D) graphical interface using both a pointing device and a keyboard.
This difference can be attributed to how assistive technologies construct a non-visual representation of the graphical interface, the overhead in the non-visual representation, and the challenges from overloading of keyboards to perform all interactions---navigation, exploration, target acquisition, performing actions (e.g., press or click), in addition to entering text.

To elaborate, assistive technologies like readers (e.g., NVDA~\cite{NVAccess38:online}, JAWS~\cite{jaws_screenshade}, and VoiceOver~\cite{voiceover_osx}), narrate onscreen content loudly in response to keyboard shortcuts. 
% 
They construct an invisible \T{DOM}~\cite{DOM2022} tree-like, textual meta-representation of an application by consuming the operating systems' built-in accessibility support, commonly known as accessible APIs~\cite{msaa_arch, ui_automation, osx_api}.
Each node in this tree is a proxy for a UI element, the  attributes of a node  contains textual descriptions (e.g., name, type) of the underlying UI element (if available), and the parent-child relationships of different nodes supposedly represent their visual semantic on the screen. 
For example, Figure~\ref{fig:hnav_illustration}.a shows the partial UI an app and Figure~\ref{fig:hnav_illustration}.b shows it  partial meta-representation tree.
% 

Often, this meta representation is  not reliable and can differ from the app's visual layout~\cite{potluri2021examining, table-view2} due to limited expressiveness in accessibility APIs (e.g., color information is not represented~\cite{harris_interoperability});
limited accessibility supports in the GUI frameworks (e.g., applications like Audacity\footnote{a popular music editing software that many blind individuals use to create music as a hobby or a profession~\cite{audacityApp}.} that are developed in a cross-platform GUI framework, such as wxWidget~\cite{wxWidgetLibrary}, have many accessibility bugs~\cite{momotaz_plugin});
and developers' lack of accessibility awareness or errors (e.g., not providing alt-text for images~\cite{guinness2018caption, ross2018, gleason2019s}, assigning incorrect metadata or attributes~\cite{momotaz_plugin}). 
% 
For example, in a web page, some UI elements may not have a meta representation if developers incorrectly assign an HTML markup, \texttt{\small aria-hidden = ``true''}, making them unreachable to screen readers. 
Also, some UI elements that belong to a same group visually, can appear in different branches in the tree due to developers' error  (see Figure~\fx{xx}).
% 
These discrepancies between an app's meta representation and graphical representation are oblivious to sighted users who can perceive its UI visually and manipulate it directly with a pointing device. 
However, these pose major accessibility and usability challenges for blind users in their screen reader-mediated interaction.
% 

Walking in this (unreliable) tree with a keyboard (i.e., navigating) is an overhead unique to blind users.  

For example, blind users can navigate (a) \textit{serially}, from left to right, top to bottom, using \T{TAB} and directional \T{Arrow} keys, or (b) \textit{hierarchically}, starting from the root node, then its children, then grand children, using a combination special shortcuts keys (e.g., \T{Control+Option+Shift+Down or Up Arrow} to get into  or out of a parent node in VoiceOver). 
% 
Both navigation strategies are cumbersome, slow, and tedious, as blind user need to navigate through an arbitrary number intermediate nodes to move their screen reader focus from a source UI to the target UI.
Prior work, for example, indicates that non-visual interaction can take up to $3\times$ more than the visual interaction~\cite{vi_difficulties, ram_prediction}.

Furthermore, overloading keyboards for all interactions is error-prone and difficult to learn.
For example, it is common to mix-up one shortcut with another, and most blind users build muscle memory with extensive practice to achieve basic proficiency~\cite{Billah_ubiquitous}.
% 
This is unfortunate because user interfaces in modern applications and web pages are rich, interactive, and carefully designed with a combination of spatial location and typographic cues, such as hierarchy, font face, color, whitespace~\cite{table-view2}---all to create an easy to perceive and easy to interact interface for sighted users.
\end{comment}







\begin{comment}
To that end, we design and develop \textbf{\emph{\sc \sysname{}}}, a mouse-shaped input device that has three identical rotary wheels and two side buttons of disproportionate size. 
%
As shown in Figure~\ref{fig:teaser}, a user rests three fingers over the three wheels to rotate each wheel individually using a single finger or simultaneously using multiple fingers. 
%
Both side buttons are thumb-accessible and their differences in size convey their roles tactilely---the big one indicates it is  the primary button, akin to the Left-click button of a mouse, which is expected to be used frequently. 
% \fixmeth{mention that \sysname{} uses haptics}
%
Similarly, the small one stands for the secondary or the Right-click button. 
%
\sysname{} primarily operates in two modes, namely \hnav{} mode and \fnav{} mode. In \hnav{} mode, as shown in Figure~\ref{fig:hnav_illustration}, BLV users can navigate UI elements in complex, hierarchical layout rapidly---using one wheel for each level of hierarchy.
% 
\fnav{} mode, as shown in Figure~\ref{fig:fnav_illustration}, enables them to move the cursor on the 2D screen non-visually with ease to target a UI element,  if instructed.
%
Users can seamlessly toggle between two modes by simultaneously pressing the two side buttons.
%
\sysname{} provides different audio-haptic feedback to convey the context of the cursor to the users.
%
The \hnav{} mode of \sysname{} is designed to address the issue of navigating tree-like hierarchies and the \fnav{} mode is designed to enable fine-grained context-aware movement of the cursor on the screen. 



Prior work indicated that people with vision impairments preferred a rotary device (e.g., a wheel, a dial) for navigation over a keyboard~\cite{Billah_speeddial, Billah_steeringwheel, haena-speeddial1, haena-speeddial2}. 
Since keyboards offer numerous shortcuts, it is easy to mix up one for the other. 
In contrast, the rotary devices support only a few gestures (e.g., rotate and press), making rotation-based interaction easy, efficient, and less error-prone. 
% 
Besides, prototypes that uses a rotary input, such a Surface Dial~\cite{surface_dial} in \textit{Speed-Dial}~\cite{Billah_speeddial} and a mouse wheel in \textit{NVMouse}~\cite{haena-speeddial2}, offer simple gestures (e.g., a single-press or a double-press) to go up and down in the hierarchical navigation. 
% 
Furthermore, since rotation is inherently a 1D operation, many blind users naturally associate rotation with moving the mouse cursor and press with clicking with the mouse~\cite{Billah_speeddial, haena-speeddial1}. 
%
Because of these encouraging results, we included rotation-based interaction in our design space.


A user study with $12$ BLV participants showed that they needed 41.3\% less time in doing tasks using Wheeler's \hnav{} mode, compared to using the combination of keyboard and SR. 
%
In addition, they were able to move the cursor around the screen to acquire targets (as instructed) using \sysname{}'s \fnav{} mode.
%
Evaluation of this feature with our participants in multiple sessions revealed that the time for locating a target on the screen improves from one session to the next.
%
This study, accompanied by a diary study with our blind co-author also revealed that \sysname{} is easy to learn and easy to use; and it offers serendipitous benefits, such as to collaborate with sighted users on a shared screen and to click on partially accessible UI elements, which are otherwise unreachable via a keyboard.


While moving a cursor using keyboard keys is feasible in some cases~\cite{windows_mouse, voiceover_touchpad}, it lacks precision, a convenient pace control mechanism, and has usability issues according to the findings of our participatory design session interviews (\S\ref{sec:design}).
%
As such, a convenient, easy, and user-adaptable mechanism is necessary for the BLV users to move the cursor on the screen. 


Another issue with SRs arise when navigating tree-like hierarchies.
Hierarchical menus (e.g., ribbons) are common in modern applications such as Microsoft Office Suite~\cite{darejeh2014investigation}. 
These hierarchies are similar to HTML DOM trees where each node in a tree is reachable from any other node.
Some SRs such as VoiceOver~\cite{voiceover_osx} and ChromeVox~\cite{chromevox} allow users to go to the child or parent of a certain menu option (i.e., node in a tree) one at a time.
However, even when two nodes are close in the visual layout of a UI, they can be under different subtrees in the hierarchy.
In such a scenario, the traversal path between the two nodes becomes lengthy and tiresome.
%

An additional challenge encountered with screen readers (SRs) pertains to navigating tree-like hierarchical structures. Hierarchical menus, exemplified by ribbons, are prevalent in contemporary applications like the Microsoft Office Suite~\cite{darejeh2014investigation}. These hierarchical structures resemble HTML Document Object Model (DOM) trees, where any node within the tree is accessible from another. Certain SRs, including VoiceOver~\cite{voiceover_osx} and ChromeVox~\cite{chromevox}, enable users to traverse the hierarchical structure by moving between the parent and child elements of a specific menu option, or node, sequentially. However, when two nodes are positioned in close proximity within the user interface's visual layout but reside under distinct subtrees in the hierarchy, the navigation path between them can become lengthy and exhausting for the user.
\end{comment}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This paper presents \textbf{\sc \sysname{}}, an input device aims to address the above challenges. The technical idea is rooted in the observations that 
% (i) travelling the DOM tree faster can improve the efficiency of non-visual interaction; 
% % 
% (2) a faster navigation can relief the users from memorizing numerous keyboard; shortcuts;
% % 
% (3) delegating certain interactions (e.g., navigation, target acquisition, performing click actions) to a separate input device can release the keyboard from overloaded with shortcuts;
% % 
% (4) an input device to take advantage of the fine motor control of human hands, especially the small muscle groups and joints in the fingers that are densely represented in the human motor and sensory cortex and can process information faster than than other body parts~\cite{zhai1996influence, mackenzie2001accuracy, bowden2016ergonomics, budnick2017ergonomics}.
% %
% (5) an awareness of mouse cursor and visual semantics are important to resolve reliability issues of the DOM tree. These can also improve blind users' navigation strategies; enable them to collaborate with sighted users, who often provide instructions with respect to the visual layout; and allow them to build their own visually-oriented artifacts (e.g., websites)~\cite{potluri2021examining}.
% 
